On The Morel Structure Conjecture

We prove that Witt K-theory is effective over any perfect field of characteristic $2$ and consequently finish the proof of the Morel structure conjecture initiated by Bachmann.

==> Setup/document_macros.tex <==
\ProvidesPackage{document_macros}


%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
% Document Macros                                                   %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%







%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
% amsart improvements                                               %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%-------------------------------------------------------------------%
% Better amsart theorem styling                                     %
%-------------------------------------------------------------------%

\makeatletter
\def\swappedhead#1#2#3{%
  \thmnumber{\@upn{\the\thm@headfont#2\@ifnotempty{#1}{\,~}}}%
  \thmname{#1}%
  \thmnote{ {\the\thm@notefont{#3}}}}
\makeatother

%-------------------------------------------------------------------%
% Better amsart section styling                                     %
%-------------------------------------------------------------------%

\makeatletter
\def\@seccntformat#1{%
  \protect\textup{\protect\@secnumfont
    \ifnum\pdfstrcmp{subsection}{#1}=0 \bfseries\fi% subsection # in \bfseries
    \csname the#1\endcsname
    \protect{\,}
  }%
}  
\makeatother

\usepackage{secdot}


%-------------------------------------------------------------------%
% Better amsart table of contents                                   %
%-------------------------------------------------------------------%

% Improves amsart table of contents
\makeatletter
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima
      \ifcase #1
       \or\or \hskip 1em \or \hskip 2em \else \hskip 3em \fi%
      #6\nobreak\relax
    \hfill\hbox to\@pnumwidth{\@tocpagenum{#7}}\par% <---- \dotfill -> \hfill
    \nobreak
    \endgroup
  \fi}
\makeatother


==> Setup/document_style.tex <==
\ProvidesPackage{document_style}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Options                                                          %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%\newif\ifminionmath
%\newif\ifnormal
%\DeclareOption{minionmath}{\minionmathtrue}
%\DeclareOption{normal}{\normaltrue}
%\ProcessOptions*

%-------------------------------------------------------------------%
%-------------------------------------------------------------------

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Standard useful packages                                         %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{etoolbox}
\usepackage{todonotes}
\usepackage{imakeidx}
\usepackage{xcolor}
\usepackage{soul}
\usepackage{nicefrac}
\usepackage{stackrel}

%\usepackage{comment}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Packages and options for collaborating                           %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\usepackage{changes} % this packages breaks \emph{} for some reason
\normalem % this command repairs \emph{}

\newcommand{\makeblack}{\color{black}}
\newcommand{\makewhite}{\color{white}}
\newcommand{\makered}{\color{red}}
\newcommand{\makeblue}{\color{blue}}
\newcommand{\makegreen}{\color{green}}
\newcommand{\makeyellow}{\color{yellow}}
\newcommand{\makecyan}{\color{cyan}}
\newcommand{\makemagenta}{\color{magenta}}

\newcommand{\black}[1]{{\makeblack #1}}
\newcommand{\white}[1]{{\makewhite #1}}
%\newcommand{\red}[1]{{\makered #1}}
\newcommand{\blue}[1]{{\makeblue #1}}
\newcommand{\green}[1]{{\makegreen #1}}
\newcommand{\yellow}[1]{{\makeyellow #1}}
\newcommand{\cyan}[1]{{\makecyan #1}}
\newcommand{\magenta}[1]{{\makemagenta #1}}

\definecolor{darklimegreen}{RGB}{31, 142, 8}
\newcommand{\makedarklimegreen}{\color{darklimegreen}}
\newcommand{\darklimegreen}[1]{{\makedarklimegreen #1}}

\definecolor{orange}{RGB}{255, 140, 0}
\newcommand{\makeorange}{\color{orange}}
\newcommand{\orange}[1]{{\makeorange #1}}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Colors                                                           %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

% Solarized
\definecolor{sbase03}{HTML}{002B36}
\definecolor{sbase02}{HTML}{073642}
\definecolor{sbase01}{HTML}{586E75}
\definecolor{sbase00}{HTML}{657B83}
\definecolor{sbase0}{HTML}{839496}
\definecolor{sbase1}{HTML}{93A1A1}
\definecolor{sbase2}{HTML}{EEE8D5}
\definecolor{sbase3}{HTML}{FDF6E3}
\definecolor{syellow}{HTML}{B58900}
\definecolor{sorange}{HTML}{CB4B16}
\definecolor{sred}{HTML}{DC322F}
\definecolor{smagenta}{HTML}{D33682}
\definecolor{sviolet}{HTML}{6C71C4}
\definecolor{sblue}{HTML}{268BD2}
\definecolor{scyan}{HTML}{2AA198}
\definecolor{sgreen}{HTML}{859900}

% Other colors
\definecolor{tulip}{RGB}{69, 9, 67}
\definecolor{love}{RGB}{128, 15, 37}
\definecolor{champ}{RGB}{249, 205, 173}
\definecolor{lobster}{RGB}{255, 64, 64}
\definecolor{dutch}{RGB}{22, 147, 165}
\definecolor{slate}{RGB}{42, 54, 59}

%\patchcmd{\section}{\normalfont}{\normalfont\color{love}}{}{}
\patchcmd{\subsection}{\normalfont}{\normalfont\color{love}}{}{}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  PDF bookmarks                                                    %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

% Adds section numbers to PDF bookmarks
\usepackage{bookmark}
\bookmarksetup{
  numbered, 
  open,
}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Hyperlinks                                                       %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\usepackage{url} % Allows for printing of URLs with TeX symbols that normally wouldn't be printed such as "~"
\usepackage{hyperref}
\hypersetup{
  colorlinks = true, %set true if you want colored links
  linktoc = all,     %set to all if you want both sections and subsections linked
  linkcolor = love,  %choose some color if you want links to stand out
  citecolor = love,
  urlcolor = slate,
  pdfencoding = unicode,
  hypertexnames = true,
  bookmarksdepth = subsubsection,
}


%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Citations                                                        %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%\usepackage{citationscheme}
%\usepackage{csquotes}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Internal references                                              %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%-------------------------------------------------------------------%
%  Packages & basic commands                                        %
%-------------------------------------------------------------------%

\setcounter{secnumdepth}{2}

\usepackage{amsthm}

% The placement of this package is IMPORTANT. (It may not work if it is placed in a different order with respect to other packages.)
\usepackage[noabbrev,nameinlink,capitalize]{cleveref} 
\newcommand{\creflastconjunction}{, and\nobreakspace} % Makes cleveref use an Oxford comma for multiple citations
% Not sure why but this seems to be introducing an error. Maybe this is no longer necessary?

%-------------------------------------------------------------------%
%  Environment names                                                %
%-------------------------------------------------------------------%

\numberwithin{equation}{section} % Aligns all numbering with the equation

\swapnumbers % Makes numbers appear before environment names

\patchcmd{\swappedhead}{(#3)}{\normalfont #3}{}{} % patch with 2 uses:
% Use 1: remove auto parenthesis in \begin{theorem}[---]
% Use 2: avoid an issue with \sffamily and theoremstyles

\theoremstyle{definition}
\newtheorem{nul}[equation]{}
\newtheorem{axiom}[equation]{Axiom}
\newtheorem{construction}[equation]{Construction}
\newtheorem{convention}[equation]{Convention}
\newtheorem{counterexample}[equation]{Counterexample}
\newtheorem{definition}[equation]{Definition}
\newtheorem{example}[equation]{Example}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{notation}[equation]{Notation}
\newtheorem{observation}[equation]{Observation}
\newtheorem{question}[equation]{Question}
\newtheorem{recollection}[equation]{Recollection}
\newtheorem{remark}[equation]{Remark}
\newtheorem{subexample}[equation]{Subexample}
\newtheorem{variant}[equation]{Variant}
\newtheorem{warning}[equation]{Warning}

\newtheorem*{acknowledgments}{Acknowledgments}
\newtheorem*{slogan*}{Slogan}

\theoremstyle{plain}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{assumption}[equation]{Assumption}
%-------------------------------------------------------------------%
%  Cleverref names                                                  %
%-------------------------------------------------------------------%

\crefname{section}{\S\!}{\S\S\!}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{\S\!}{\S\S\!}
\Crefname{subsection}{Subsection}{Subsections}

\crefformat{nul}{(#2#1#3)} % Has cref parenthesize "nul" references
\crefname{nul}{}{}
\Crefformat{nul}{(#2#1#3)}
\Crefname{nul}{}{}

\crefname{axiom}{Axiom}{Axioms}
\Crefname{axiom}{Axiom}{Axioms}
\crefname{convention}{Convention}{Conventions}
\Crefname{convention}{Convention}{Conventions}
\crefname{conjecture}{Conjecture}{Conjectures}
\Crefname{conjecture}{Conjecture}{Conjectures}
\crefname{construction}{Construction}{Constructions}
\Crefname{construction}{Construction}{Constructions}
\crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{counterexample}{Counterexample}{Counterexamples}
\Crefname{counterexample}{Counterexample}{Counterexamples}
\crefname{definition}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}
\crefname{example}{Example}{Examples}
\Crefname{example}{Example}{Examples}
\crefname{exercise}{Exercise}{Exercises}
\Crefname{exercise}{Exercise}{Exercises}
\crefname{lemma}{Lemma}{Lemmas} 
\Crefname{lemma}{Lemma}{Lemmas} 
\crefname{notation}{Notation}{Notations}
\Crefname{notation}{Notation}{Notations}
\crefname{observation}{Observation}{Observations}
\Crefname{observation}{Observation}{Observations}
\crefname{proposition}{Proposition}{Propositions}
\Crefname{proposition}{Proposition}{Propositions}
\crefname{question}{Question}{Questions}
\Crefname{question}{Question}{Questions}
\crefname{recollection}{Recollection}{Recollections}
\Crefname{recollection}{Recollection}{Recollections}
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}
\crefname{subexample}{Subexample}{Subexamples}
\Crefname{subexample}{Subexample}{Subexamples}
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{variant}{Variant}{Variants}
\Crefname{variant}{Variant}{Variants}
\crefname{warning}{Warning}{Warnings}
\Crefname{warning}{Warning}{Warnings}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Enumerate environments                                           %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

% for easy referencing of enumerated lists
\usepackage[shortlabels]{enumitem}
\setlist[enumerate]{
     itemsep  = 0.2cm,
       label  = {\upshape (\arabic*)},
         ref  = \arabic*,
    leftmargin  = *
}

\newcommand{\stlabel}[1]{{\upshape (\ref*{#1}.\arabic*)}}

\newcommand{\enumref}[2]{{\upshape (\hyperref[#1.#2]{\ref*{#1}.\ref*{#1.#2}})}}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Font-specific packages                                           %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%\ifminionmath
%  \usepackage{minionfonts}
%\fi

%\ifnormal
%  \usepackage{normalfonts}
%\fi

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Kerning and spacing                                              %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\usepackage{xspace}

\frenchspacing

\usepackage[final,factor=1100,stretch=10,shrink=10]{microtype}

\SetProtrusion{encoding={*},family={bch},series={*},size={6,7}}
              {1={ ,750},2={ ,500},3={ ,500},4={ ,500},5={ ,500},
               6={ ,500},7={ ,600},8={ ,500},9={ ,500},0={ ,500}}

\SetExtraKerning[unit=space]
    {encoding={*}, family={bch}, series={*}, size={footnotesize,small,normalsize}}
    {\textendash={400,400},   % en-dash, add more space around it
     "28={ ,150},     % left bracket, add space from right
     "29={150, },     % right bracket, add space from left
     \textquotedblleft={ ,150},   % left quotation mark, space from right
     \textquotedblright={150, }}  % right quotation mark, space from left

\SetTracking{encoding={*}, shape=sc}{40}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Diagrams & commutative diagrams                                  %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\usepackage{tikz-cd}
\usepackage{quiver}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Standard macros                                                  %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

%\ifminionmath
 % \usepackage[minionmath]{standard_macros}
%\fi

%\ifnormal
%  \usepackage[normal]{standard_macros}
%\fi


%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Long arrows                                               %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%https://tex.stackexchange.com/questions/170592/how-to-use-leftrightarrows

\newcommand{\leftrarrows}{\mathrel{\raise.75ex\hbox{\oalign{%
  $\scriptstyle\leftarrow$\cr
  \vrule width0pt height.5ex$\hfil\scriptstyle\relbar$\cr}}}}
\newcommand{\lrightarrows}{\mathrel{\raise.75ex\hbox{\oalign{%
  $\scriptstyle\relbar$\hfil\cr
  $\scriptstyle\vrule width0pt height.5ex\smash\rightarrow$\cr}}}}
\newcommand{\Rrelbar}{\mathrel{\raise.75ex\hbox{\oalign{%
  $\scriptstyle\relbar$\cr
  \vrule width0pt height.5ex$\scriptstyle\relbar$}}}}
\newcommand{\longleftrightarrows}{\leftrarrows\joinrel\Rrelbar\joinrel\lrightarrows}

\makeatletter
\def\leftrightarrowsfill@{\arrowfill@\leftrarrows\Rrelbar\lrightarrows}
\newcommand{\xleftrightarrows}[2][]{\ext@arrow 3399\leftrightarrowsfill@{#1}{#2}}
\makeatother

\newcommand{\longrightleftarrows}{\mathrel{\substack{\longrightarrow\\[-1pt] \longleftarrow}}}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Semantic aliases                                                 %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\newcommand{\defn}{\smallcaps}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Symbol preferences                                               %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\emptyset}{\varnothing}

==> Setup/special_commands.tex <==
\ProvidesPackage{special_commands}

%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Options                                                          %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%

\newif\ifminionmath
\newif\ifnormal
\DeclareOption{minionmath}{\minionmathtrue}
\DeclareOption{normal}{\normaltrue}
\ProcessOptions*

%-------------------------------------------------------------------%
% Define                                                            %
%-------------------------------------------------------------------%
\newcommand{\name}[1]{\textsc{#1}}

%-------------------------------------------------------------------%
%  Elements of grammar in math mode                                 %
%-------------------------------------------------------------------%

\newcommand{\andeq}{\text{\qquad and\qquad}}

\newcommand{\comma}{\rlap{\ ,}}
\newcommand{\period}{\rlap{\ .}}
\newcommand{\semicolon}{\rlap{\ ;}}


%-------------------------------------------------------------------%
% (Co)limits                                                        %
%-------------------------------------------------------------------%

\newcommand{\cofib}{\ensuremath{\textup{cofib}}}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator*{\colim}{colim}
\newcommand{\fib}{\ensuremath{\textup{fib}}}
%\DeclareMathOperator{\ker}{ker}
%\DeclareMathOperator*{\lim}{lim}

%-------------------------------------------------------------------%
% 1-letter operators                                                %
%-------------------------------------------------------------------%

\DeclareMathOperator{\Nerve}{N}
\DeclareMathOperator{\trun}{\uptau}

%-------------------------------------------------------------------%
% Operators with accents                                            %
%-------------------------------------------------------------------%

\newcommand{\Cech}{\check{\mathrm{C}}}
\newcommand{\Hcech}{\check{\mathrm{H}}}

%\if@minionmath
%    \DeclareMathOperator{\et}{\acute et}
%    \DeclareMathOperator{\fet}{f \acute et}
%    \DeclareMathOperator{\proet}{pro \acute et}
%\fi

%\if@normal
%    \DeclareMathOperator{\et}{\acute et}
%    \DeclareMathOperator{\fet}{f\acute et}
%    \DeclareMathOperator{\proet}{pro\acute et}
%\fi

\DeclareMathOperator{\et}{\acute et}
\DeclareMathOperator{\fet}{f \acute et}
\DeclareMathOperator{\proet}{pro \acute et}


%-------------------------------------------------------------------%
%  Delimiters                                                       %
%-------------------------------------------------------------------% 

\newcommand{\llbracket}{\lBrack}
\newcommand{\rrbracket}{\rBrack}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ang}[1]{\langle #1 \rangle}




%-------------------------------------------------------------------%
%-------------------------------------------------------------------%
%  Variable names                                                   %
%-------------------------------------------------------------------%
%-------------------------------------------------------------------%


%MATHRM Upright Roman
\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmZ}{\mathrm{Z}}


%MATHBF Bold Roman
\newcommand\bfA{\mathbf{A}}
\newcommand\bfB{\mathbf{B}}
\newcommand\bfC{\mathbf{C}}
\newcommand\bfD{\mathbf{D}}
\newcommand\bfE{\mathbf{E}}
\newcommand\bfF{\mathbf{F}}
\newcommand\bfG{\mathbf{G}}
\newcommand\bfH{\mathbf{H}}
\newcommand\bfI{\mathbf{I}}
\newcommand\bfJ{\mathbf{J}}
\newcommand\bfK{\mathbf{K}}
\newcommand\bfL{\mathbf{L}}
\newcommand\bfM{\mathbf{M}}
\newcommand\bfN{\mathbf{N}}
\newcommand\bfO{\mathbf{O}}
\newcommand\bfP{\mathbf{P}}
\newcommand\bfQ{\mathbf{Q}}
\newcommand\bfR{\mathbf{R}}
\newcommand\bfS{\mathbf{S}}
\newcommand\bfT{\mathbf{T}}
\newcommand\bfU{\mathbf{U}}
\newcommand\bfV{\mathbf{V}}
\newcommand\bfW{\mathbf{W}}
\newcommand\bfX{\mathbf{X}}
\newcommand\bfY{\mathbf{Y}}
\newcommand\bfZ{\mathbf{Z}}
\newcommand\bfOne{\mathbf{1}}

%MATHCAL Caligraphic
\newcommand\calA{\mathcal{A}}
\newcommand\calB{\mathcal{B}}
\newcommand\calC{\mathcal{C}}
\newcommand\calD{\mathcal{D}}
\newcommand\calE{\mathcal{E}}
\newcommand\calF{\mathcal{F}}
\newcommand\calG{\mathcal{G}}
\newcommand\calH{\mathcal{H}}
\newcommand\calI{\mathcal{I}}
\newcommand\calJ{\mathcal{J}}
\newcommand\calK{\mathcal{K}}
\newcommand\calL{\mathcal{L}}
\newcommand\calM{\mathcal{M}}
\newcommand\calN{\mathcal{N}}
\newcommand\calO{\mathcal{O}}
\newcommand\calP{\mathcal{P}}
\newcommand\calQ{\mathcal{Q}}
\newcommand\calR{\mathcal{R}}
\newcommand\calS{\mathcal{S}}
\newcommand\calT{\mathcal{T}}
\newcommand\calU{\mathcal{U}}
\newcommand\calV{\mathcal{V}}
\newcommand\calW{\mathcal{W}}
\newcommand\calX{\mathcal{X}}
\newcommand\calY{\mathcal{Y}}
\newcommand\calZ{\mathcal{Z}}

%MATHSCR Script
\newcommand\scrA{\mathscr{A}}
\newcommand\scrB{\mathscr{B}}
\newcommand\scrC{\mathscr{C}}
\newcommand\scrD{\mathscr{D}}
\newcommand\scrE{\mathscr{E}}
\newcommand\scrF{\mathscr{F}}
\newcommand\scrG{\mathscr{G}}
\newcommand\scrH{\mathscr{H}}
\newcommand\scrI{\mathscr{I}}
\newcommand\scrJ{\mathscr{J}}
\newcommand\scrK{\mathscr{K}}
\newcommand\scrL{\mathscr{L}}
\newcommand\scrM{\mathscr{M}}
\newcommand\scrN{\mathscr{N}}
\newcommand\scrO{\mathscr{O}}
\newcommand\scrP{\mathscr{P}}
\newcommand\scrQ{\mathscr{Q}}
\newcommand\scrR{\mathscr{R}}
\newcommand\scrS{\mathscr{S}}
\newcommand\scrT{\mathscr{T}}
\newcommand\scrU{\mathscr{U}}
\newcommand\scrV{\mathscr{V}}
\newcommand\scrW{\mathscr{W}}
\newcommand\scrX{\mathscr{X}}
\newcommand\scrY{\mathscr{Y}}
\newcommand\scrZ{\mathscr{Z}}

%MATHFRAK Fraktur for uppercase letters
\newcommand\frakA{\mathfrak{A}}
\newcommand\frakB{\mathfrak{B}}
\newcommand\frakC{\mathfrak{C}}
\newcommand\frakD{\mathfrak{D}}
\newcommand\frakE{\mathfrak{E}}
\newcommand\frakF{\mathfrak{F}}
\newcommand\frakG{\mathfrak{G}}
\newcommand\frakH{\mathfrak{H}}
\newcommand\frakI{\mathfrak{I}}
\newcommand\frakJ{\mathfrak{J}}
\newcommand\frakK{\mathfrak{K}}
\newcommand\frakL{\mathfrak{L}}
\newcommand\frakM{\mathfrak{M}}
\newcommand\frakN{\mathfrak{N}}
\newcommand\frakO{\mathfrak{O}}
\newcommand\frakP{\mathfrak{P}}
\newcommand\frakQ{\mathfrak{Q}}
\newcommand\frakR{\mathfrak{R}}
\newcommand\frakS{\mathfrak{S}}
\newcommand\frakT{\mathfrak{T}}
\newcommand\frakU{\mathfrak{U}}
\newcommand\frakV{\mathfrak{V}}
\newcommand\frakW{\mathfrak{W}}
\newcommand\frakX{\mathfrak{X}}
\newcommand\frakY{\mathfrak{Y}}
\newcommand\frakZ{\mathfrak{Z}}

%MATHFRAK Fraktur for lowercase letters
\newcommand\fraka{\mathfrak{a}}
\newcommand\frakb{\mathfrak{b}}
\newcommand\frakc{\mathfrak{c}}
\newcommand\frakd{\mathfrak{d}}
\newcommand\frake{\mathfrak{e}}
\newcommand\frakf{\mathfrak{f}}
\newcommand\frakg{\mathfrak{g}}
\newcommand\frakh{\mathfrak{h}}
\newcommand\fraki{\mathfrak{i}}
\newcommand\frakj{\mathfrak{j}}
\newcommand\frakk{\mathfrak{k}}
\newcommand\frakl{\mathfrak{l}}
\newcommand\frakm{\mathfrak{m}}
\newcommand\frakn{\mathfrak{n}}
\newcommand\frako{\mathfrak{o}}
\newcommand\frakp{\mathfrak{p}}
\newcommand\frakq{\mathfrak{q}}
\newcommand\frakr{\mathfrak{r}}
\newcommand\fraks{\mathfrak{s}}
\newcommand\frakt{\mathfrak{t}}
\newcommand\fraku{\mathfrak{u}}
\newcommand\frakv{\mathfrak{v}}
\newcommand\frakw{\mathfrak{w}}
\newcommand\frakx{\mathfrak{x}}
\newcommand\fraky{\mathfrak{y}}
\newcommand\frakz{\mathfrak{z}}

% LOWER SHRIEK  
\newcommand{\lowershriek}{_{\shriek}}


% UPPER SHRIEK
\newcommand{\uppershriek}{^{\shriek}}


% NAMED OBJECTS
\DeclareMathOperator{\Ab}{\mathbf{Ab}}
\DeclareMathOperator{\Ani}{\mathbf{Ani}}
\DeclareMathOperator{\Spectra}{\mathbf{Sp}}
\DeclareMathOperator{\Spc}{\mathbf{Spc}}
\DeclareMathOperator{\SH}{\mathbf{SH}}
\DeclareMathOperator{\SHeff}{\mathbf{SH}^{eff}}
\DeclareMathOperator{\SHveff}{\mathbf{SH}^{veff}}
\DeclareMathOperator{\Shv}{\mathrm{Shv}}

\newcommand{\SHeffx}[1]{\mathbf{SH}{(#1)}^{\mathrm{eff}}}
\newcommand{\SHveffx}[1]{\mathbf{SH}{(#1)}^{\mathrm{veff}}}

\DeclareMathOperator{\Smk}{\mathrm{Sm}_k}
\DeclareMathOperator{\essSmk}{\mathrm{Sm}^{ess}_k}
\DeclareMathOperator{\tSmk}{\mathrm{Sm}_k^{Sm_s}}

\DeclareMathOperator{\CAlg}{\mathrm{CAlg}}
\DeclareMathOperator{\Spec}{\mathrm{Spec}} 

\DeclareMathOperator{\Sphere}{\bfS} %Sphere Spectrum




\DeclareMathOperator{\HZ}{\rmH\bfZ}
\DeclareMathOperator{\HWZ}{\rmH_W\bfZ}
\DeclareMathOperator{\HZtilde}{\widetilde{\rmH\bfZ}}

\DeclareMathOperator{\Gm}{\mathbf{G}_m}

\DeclareMathOperator{\K}{\bfK} %K-theory
\DeclareMathOperator{\KH}{\bfK\bfH} %homotopy K-theory
\DeclareMathOperator{\KGL}{\bfK \bfG \bfL} %Spectrum associated with KH inside SH
\DeclareMathOperator{\KO}{\bfK \bfO} %Hermitian K-theory
\DeclareMathOperator{\KU}{\bfK \bfU} %Complex K-theory

%-------------------------------------------------------------------%
%  AAAAA                                                       %
%-------------------------------------------------------------------% 

\DeclareMathOperator{\Fun}{\mathrm{Fun}} 
\DeclareMathOperator{\Hom}{\mathrm{Hom}} 
\DeclareMathOperator{\Map}{\mathrm{Map}} 

\newcommand{\FilS}[1]{\mathrm{Fil}^{#1}_{\mathrm{slice}}}



